Controlling Translation Formality Using Pre-trained Multilingual Language Models

This paper describes the University of Maryland's submission to the Special Task on Formality Control for Spoken Language Translation at \iwslt, which evaluates translation from English into 6 languages with diverse grammatical formality markers. We investigate to what extent this problem can be addressed with a \textit{single multilingual model}, simultaneously controlling its output for target language and formality. Results show that this strategy can approach the translation quality and formality control achieved by dedicated translation models. However, the nature of the underlying pre-trained language model and of the finetuning samples greatly impact results.

==> tables/parameters.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\centering
\begin{tabular}{lll}
\toprule
Model            & Parameters/model & \# models \\ \midrule
Baseline (en-de) & 314M          & 2                            \\
Baseline (en-es) & 314M          & 2                            \\ 
Baseline (en-ja) & 316M          & 2                            \\ 
Baseline (en-hi) & 314M          & 2                            \\ 
Baseline (en-it) & 314M          & 1                            \\ 
Baseline (en-ru) & 314M          & 1                            \\ \midrule
Additive mT5     &  1250M                    & 1                            \\ \midrule
Additive mBART   &    610M              & 1                            \\ \bottomrule
\end{tabular}
\caption{Number of parameters for each architecture, demarcated to reflect the groups required to cover the entire test set. \sa{This can be made super compact either in text or reported in offical/unofficial results.}}
\label{tab:capacity} 
\end{table}
